Smooth Normalizing Flows

Normalizing flows are a promising tool for modeling probability distributions in physical systems. While state-of-the-art flows accurately approximate distributions and energies, applications in physics additionally require smooth energies to compute forces and higher-order derivatives. Furthermore, such densities are often defined on non-trivial topologies. A recent example are Boltzmann Generators for generating 3D-structures of peptides and small proteins. These generative models leverage the space of internal coordinates (dihedrals, angles, and bonds), which is a product of hypertori and compact intervals. In this work, we introduce a class of smooth mixture transformations working on both compact intervals and hypertori. Mixture transformations employ root-finding methods to invert them in practice, which has so far prevented bi-directional flow training. To this end, we show that parameter gradients and forces of such inverses can be computed from forward evaluations via the inverse function theorem. We demonstrate two advantages of such smooth flows: they allow training by force matching to simulation data and can be used as potentials in molecular dynamics simulations.

==> dumpster.tex <==
\subsection{Differentiation through Blackbox Root-Finding}

\paragraph{Gradient relations}
Here we derive the gradient relations as discussed in Sec. \ref{sec:black-box-inverse-optimization}. This is a generalization of the usual inverse function theorem in 1D to the case of scalar bijections conditioned on some parameter $\bm \theta$. For reasons of brevity in the main text and precision in the proof, we used a different notation in Sec. \ref{sec:black-box-inverse-optimization} than we will use here. 
\begin{theorem}
\label{thm:backward-gradients}
Let 
\begin{align*}
    \alpha \colon (x; \bm \theta) \mapsto y; \qquad
    \beta \colon (y; \bm \theta) \mapsto x
\end{align*}
be $\mathcal{C}^{2}$ functions satisfying
\begin{align} \label{eq:inverse-condition}
    \alpha(\beta(y; \bm \theta); \bm \theta) = y; \qquad
    \beta(\alpha(x; \bm \theta); \bm \theta) = x
\end{align}
and 
\begin{align}
    \partial_{x} \alpha(x; \bm \theta) > 0; \qquad
    \partial_{y} \beta(y; \bm \theta) > 0.
\end{align}
Let further
\begin{align}
    g_{\alpha}(x,\bm \theta) = \log \left| \frac{\partial \alpha(x; \bm \theta) }{\partial x } \right|; \quad g_{\beta}(y,\bm u) = \log \left| \frac{\partial \beta(y; \bm u) }{\partial y } \right|.
\end{align}
For $y = \alpha(x; \bm \theta)$, we have the following gradient relations
\begin{align}
    \frac{\partial \beta(y; \bm \theta)}{\partial y} &= \left(\frac{\partial \alpha(x; \bm \theta)}{\partial x}\right)^{-1} \label{eq:grad-out-in} \\
    \frac{\partial \beta(y; \bm \theta)}{\partial \bm \theta} &= - \left(\frac{\partial \alpha(x; \bm \theta)}{\partial x}\right)^{-1} \frac{\partial \alpha(x; \bm \theta)}{\partial \bm \theta} \label{eq:grad-out-param} \\
    \frac{\partial g_{\beta}(y; \bm \theta)}{\partial y} &= - \left(\frac{\partial \alpha(x; \bm \theta)}{\partial x}\right)^{-1} \frac{\partial g_{\alpha}(x; \bm \theta)}{\partial x} \label{eq:grad-density-in} \\
    \frac{\partial g_{\beta}(y; \bm \theta)}{\partial \bm \theta} &= \left(\frac{\partial \alpha(y; \bm \theta)}{\partial x}\right)^{-1} \left(  \frac{\partial g_{\alpha}(x; \bm \theta)}{\partial x} \frac{\partial \alpha(x; \bm \theta)}{\partial \bm \theta} - \frac{\partial^{2} \alpha(x; \bm \theta)}{\partial \bm \theta \partial x} \right) \label{eq:grad-density-param}
\end{align}
\end{theorem}
\begin{proof}
    We have
    \begin{align}
        \frac{d}{d x} \beta(\alpha(x; \bm \theta); \bm \theta) = \frac{\partial \beta(\alpha(x; \bm \theta); \bm \theta)}{\partial y} \frac{\partial \alpha(x; \bm \theta)}{\partial x} = \frac{d x}{d x} = 1.
    \end{align}
    and thus
    \begin{align}
        \frac{\partial \beta(\alpha(x; \bm \theta); \bm \theta)}{\partial y}  &= \left( \frac{\partial \alpha(x; \bm \theta)}{\partial x} \right)^{-1}.
    \end{align}
    
    Now 
    \begin{align}
        \frac{d}{d \bm \theta} \beta(\alpha(x; \bm \theta); \bm \theta) = \frac{\partial \beta(\alpha(x; \bm \theta); \bm \theta)}{\partial y} \frac{\partial \alpha(x; \bm \theta)}{\partial \bm \theta} + \frac{\partial \beta(\alpha(x; \bm \theta); \bm \theta)}{\partial \bm \theta} = \frac{\partial x}{\partial \bm \theta} = 0.
    \end{align}
    which gives
    \begin{align}
        \frac{\partial \beta(\alpha(x; \bm \theta); \bm \theta)}{\partial \bm \theta} 
        &= \frac{\partial \beta(\alpha(x; \bm \theta); \bm \theta)}{\partial y} \frac{\partial \alpha(x; \bm \theta)}{\partial \bm \theta}\\
        &= \left( \frac{\partial \alpha(x; \bm \theta)}{\partial x} \right)^{-1} \frac{\partial \alpha(x; \bm \theta)}{\partial \bm \theta}
    \end{align}
    
    Combining
    \begin{align}
        \frac{d }{d x} \frac{d }{d x} \beta(\alpha(x; \bm \theta); \bm \theta) &= \frac{d }{d x} \frac{d x}{d x} = 0
    \end{align}
    and 
    \begin{align}
        \frac{d }{d x} \frac{d }{d x} \beta(\alpha(x; \bm \theta); \bm \theta) &= \frac{d}{dx} \frac{\partial \beta(\alpha(x; \bm \theta); \bm \theta)}{\partial y} \frac{\partial \alpha(x; \bm \theta)}{\partial x} \\
        &= \frac{\partial^{2} \beta(\alpha(x; \bm \theta); \bm \theta)}{\partial y\partial y} \left(\frac{\partial \alpha(x; \bm \theta)}{\partial x} \right)^{2} + \frac{\partial \beta(\alpha(x; \bm \theta); \bm \theta)}{\partial y} \frac{\partial^{2} \alpha(x; \bm \theta)}{\partial x \partial x} 
    \end{align}
    we obtain
    \begin{align}
    \frac{\partial^{2} \beta(\alpha(x; \bm \theta); \bm \theta)}{\partial y \partial y}
          &= - \left(\frac{\partial \alpha(x; \bm \theta)}{\partial x} \right)^{-2} \frac{\partial \beta(\alpha(x; \bm \theta); \bm \theta)}{\partial y} \frac{\partial^{2} \alpha(x; \bm \theta)}{\partial x \partial x} \\
          &= - \left(\frac{\partial \alpha(x; \bm \theta)}{\partial x} \right)^{-3} \frac{\partial^{2} \alpha(x; \bm \theta)}{\partial x \partial x}\\
          &= - \left(\frac{\partial \alpha(x; \bm \theta)}{\partial x} \right)^{-2} \frac{\partial}{\partial x} \log \left ( \frac{\partial \alpha(x; \bm \theta)}{\partial x}  \right)\\
          &= - \left(\frac{\partial \alpha(x; \bm \theta)}{\partial x} \right)^{-2} \frac{\partial g_{\alpha}(x; \bm \theta)}{\partial x}
    \end{align}
    and thus
    \begin{align}
        \frac{\partial}{\partial y} g_{\beta}(\alpha(x; \bm \theta); \bm \theta) 
        &= \left(\frac{\partial \beta(\alpha(x; \bm \theta); \bm \theta)}{\partial y} \right)^{-1} \frac{\partial^{2} \beta(\alpha(x; \bm \theta); \bm \theta)}{\partial y \partial y} \\
        &= - \left(\frac{\partial \alpha(x; \bm \theta)}{\partial x} \right)^{-1} \frac{\partial g_{\alpha}(x; \bm \theta)}{\partial x}
    \end{align}
    Finally, combining
    \begin{align}
        \frac{d }{d \bm \theta} \frac{d }{d x} \beta(\alpha(x; \bm \theta); \bm \theta)  &= \frac{d }{d \bm \theta} \frac{d x}{d x} = 0
    \end{align}
    and
    \begin{align}
        \frac{d }{d \bm \theta} \frac{d }{d x} \beta(\alpha(x; \bm \theta); \bm \theta) 
        &= \frac{d}{d\bm \theta} \frac{\partial \beta(\alpha(x; \bm \theta); \bm \theta)}{\partial y} \frac{\partial \alpha(x; \bm \theta)}{\partial x} \\
        &= \frac{\partial^{2} \beta(\alpha(x; \bm \theta); \bm \theta)}{\partial y\partial y} \frac{\partial \alpha(x; \bm \theta)}{\partial \bm \theta} \frac{\partial \alpha(x; \bm \theta)}{\partial x}  \\
        &\quad + \frac{\partial \beta(\alpha(x; \bm \theta); \bm \theta)}{\partial y} \frac{\partial^{2} \alpha(x; \bm \theta)}{\partial \bm \theta \partial x} \nonumber  \\
        &\quad + \frac{\partial^{2} \beta(\alpha(x; \bm \theta); \bm \theta)}{\partial \bm \theta  \partial y} \frac{\partial \alpha(x; \bm \theta)}{\partial x} \nonumber 
    \end{align}
    gives us
    \begin{align}
        \frac{\partial^{2}\beta(\alpha(x; \bm \theta); \bm \theta)}{\partial \bm \theta \partial y}
        &= - \frac{\partial^{2} \beta(\alpha(x; \bm \theta); \bm \theta)}{\partial y\partial y} \frac{\partial \alpha(x; \bm \theta)}{\partial \bm \theta} \\
        &\quad - \frac{\partial \beta(\alpha(x; \bm \theta); \bm \theta)}{\partial y} \frac{\partial^{2} \alpha(x; \bm \theta)}{\partial \bm \theta \partial x} \left(\frac{\partial \alpha(x; \bm \theta)}{\partial x}\right)^{-1} \nonumber \\
        &= \left(\frac{\partial \alpha(x; \bm \theta)}{\partial x} \right)^{-2} \frac{\partial g_{\alpha}(x; \bm \theta)}{\partial x} \frac{\partial \alpha(x; \bm \theta)}{\partial \bm \theta} \\
        &\quad - \left(\frac{\partial \alpha(x; \bm \theta)}{\partial x} \right)^{-2} \frac{\partial^{2} \alpha(x; \bm \theta)}{\partial \bm \theta \partial x}  \nonumber\\
        &= \left(\frac{\partial \alpha(x; \bm \theta)}{\partial x} \right)^{-2} \left(\frac{\partial g_{\alpha}(x; \bm \theta)}{\partial x} \frac{\partial \alpha(x; \bm \theta)}{\partial \bm \theta}  - \frac{\partial^{2} \alpha(x; \bm \theta)}{\partial \bm \theta \partial x} \right)
    \end{align}
    And thus we get
    \begin{align}
        \frac{\partial}{\partial \bm \theta} g_{\beta}(\alpha(x; \bm \theta); \bm \theta) 
        &= \left( \frac{\partial \beta(\alpha(x; \bm \theta); \bm \theta)}{\partial y}  \right)^{-1} \frac{\partial^{2}\beta(\alpha(x; \bm \theta); \bm \theta)}{\partial \bm \theta \partial y} \\
        &= \left(\frac{\partial \alpha(x; \bm \theta)}{\partial x} \right)^{-1} \left(\frac{\partial g_{\alpha}(x; \bm \theta)}{\partial x} \frac{\partial \alpha(x; \bm \theta)}{\partial \bm \theta}  - \frac{\partial^{2} \alpha(x; \bm \theta)}{\partial \bm \theta \partial x} \right)
    \end{align}
\end{proof}

\paragraph{Additional derivations for forces}

\begin{align}
    d^3_{x} \beta 
    &= d_{x} \left( 
        \partial_{y}^{2} \beta \left(\partial_{x} \alpha \right)^2 
        + \partial_{y} \beta \partial_{x}^{2} \alpha 
    \right) \\
    &= \partial_{y}^{3} \beta \left(\partial_{x} \alpha \right)^3 
    + 2  \partial_{y}^{2} \beta \partial_{x} \alpha \partial^2_{x} \alpha
    + \partial^2_{y} \beta \partial_{x} \alpha \partial_{x}^{2} \alpha
    + \partial_{y} \beta \partial_{x}^{3} \alpha\\
    &= \partial_{y}^{3} \beta \left(\partial_{x} \alpha \right)^3 
    + 3  \partial_{y}^{2} \beta \partial_{x} \alpha \partial^2_{x} \alpha
    + \partial_{y} \beta \partial_{x}^{3} \alpha = 0\\
    \implies&\\
    \partial_{y}^{3} \beta &= -\left(\partial_{x} \alpha \right)^{-3}\left[ 3  \partial_{y}^{2} \beta \partial_{x} \alpha \partial^2_{x} \alpha
    + \partial_{y} \beta \partial_{x}^{3} \alpha \right] \\
     &= -\left(\partial_{x} \alpha \right)^{-4}\left[ 3   \partial_{x} g_{\alpha}   \partial^2_{x} \alpha
    + \partial_{x}^{3} \alpha \right] \\
\end{align}

\begin{align}
    d_{\bm \theta} d^2_{x} \beta 
    &= d_{\bm \theta} \left( 
        \partial_{y}^{2} \beta \left(\partial_{x} \alpha \right)^2 
        + \partial_{y} \beta \partial_{x}^{2} \alpha 
    \right) \\
    &= 
        \partial_{\bm \theta} \partial_{y}^{2} \beta \left(\partial_{x} \alpha \right)^2 
        + \partial_{y}^{3} \beta  \partial_{\bm \theta} \alpha \left(\partial_{x} \alpha \right)^2 
        + \partial_{y}^{2} \beta 2 \left(\partial_{x} \alpha \right) \partial_{\bm \theta} \partial_{x} \alpha
        \\ &\quad
        + \partial_{\bm \theta} \partial_{y} \beta \partial_{x}^{2} \alpha 
        + \partial^2_{y} \beta \partial_{\bm \theta} \alpha \partial_{x}^{2} \alpha 
        + \partial_{y} \beta \partial_{\bm \theta} \partial_{x}^{2} \alpha = 0
     \\
    \implies&\\
    \partial_{\bm \theta} \partial_{y}^{2} \beta &= - \left(\partial_{x} \alpha \right)^{-2} \Bigg[ 
        \partial_{y}^{3} \beta  \partial_{\bm \theta} \alpha \left(\partial_{x} \alpha \right)^2 
        + \partial_{y}^{2} \beta 2 \left(\partial_{x} \alpha \right) \partial_{\bm \theta} \partial_{x} \alpha
        \\ &\qquad\qquad\qquad
        + \partial_{\bm \theta} \partial_{y} \beta \partial_{x}^{2} \alpha 
        + \partial^2_{y} \beta \partial_{\bm \theta} \alpha \partial_{x}^{2} \alpha 
        + \partial_{y} \beta \partial_{\bm \theta} \partial_{x}^{2} \alpha
    \Bigg] 
\end{align}
